Constraining the doability of relativistic quantum tasks

We show within the framework of relativistic quantum tasks that the doability of any task is fully determined by a small subset of its parameters that we call its "coarse causal structure", as well as the distributed computation it aims to accomplish. We do this by making rigorous the notion of a protocol using a structure known as a spacetime circuit, which describes how a computation is preformed across a region of spacetime. Using spacetime circuits we show that any protocol that can accomplish a given task can, without changing its doability, undergo significant geometric modifications such as changing the background spacetime and moving the location of input and output points, so long as the coarse causal structure of the task is maintained. Besides giving a powerful tool for determining the doability of a task, our results strengthen the no-go theorem for position based quantum cryptography to include arbitrary sending and receiving of signals by verifier agents outside the authentication region. They also serve as a consistency check for the holographic principle by showing that discrepancies between bulk and boundary causal structure can not cause a task to be doable in one but not the other.

==> Scraps.tex <==
\subsubsection{Local symplectic rotations}
Consider a local basis change on individual system modes. For this basis change to preserve Gaussianity, it must act as a symplectic rotation on the system states and operators. Since for many calculations we will assume that the system will begin in its ground state, which is symmetric under local symplectic rotations of the system modes, the effect of such a basis change is simply the transformation
\begin{align*}
  \hat{\textbf{X}}_{S,1}\rightarrow R_1(\theta)\hat{\textbf{X}}_{S,1}\\ 
  \hat{\textbf{X}}_{S,1}\rightarrow R_2(\theta)\hat{\textbf{X}}_{S,1}
\end{align*}
for some $R_1,R_2\in SO(2)$ acting on the symplectic space. Recalling that the form of the interaction Hamiltonian is,
\be
H_{SA}=\frac{1}{2}\hat{\textbf{X}}^\top_{S,1}h\hat{\textbf{X}}_{A,1}+\frac{1}{2}\hat{\textbf{X}}^\top_{S,2}g\hat{\textbf{X}}_{A,2}
\ee
we see that, as far as the dynamics are concerned, these transformations are trivially equivalent to
\begin{align}
    \hat{\textbf{X}}_{S,1}\rightarrow R_1(\theta)\hat{\textbf{X}}_{S,1} \Leftrightarrow h\rightarrow R_1^\top(\theta)h\\
    \hat{\textbf{X}}_{S,2}\rightarrow R_2(\theta)\hat{\textbf{X}}_{S,1} \Leftrightarrow g\rightarrow R_2^\top(\theta)g.
\end{align}
Writing 
\be
R_1(\theta)=\begin{pmatrix}
\cos(\theta) & -\sin(\theta)\\
\sin(\theta) & \cos(\theta)
\end{pmatrix}=\cos(\theta)\mathds{1}-\sin(\theta)\omega
\ee

\kfir{NOt DONE!}


\subsubsection{Constraints}
A time evolution operator generated by a Hamiltonian of the form
\begin{equation}\label{eq:nonentanglinghamiltonian}
    H=\hat{O}_{S_1}\otimes \hat{O}_{A_1}+\hat{O}_{S_2}\otimes \hat{O}_{A_2}
\end{equation}
with $\hat{O}$ some operators acting on the space denoted by their subscript, can not create entanglement between $S_1$ and $S_2$. The proof, which is similar to one given in \cite{Simidzija}, goes as follows:
The state of the system and ancilla at $t=0$ is given by some $\rho=\rho_{A_1,A_2}\otimes\rho_{S_1}\otimes\rho_{S_2}$. At time $t$, the state of the system is given by
\begin{align*}
    \rho_{S_1,S_2}(t)=\Tr_{A_1,A_2}[U_1U_2\rho_{A_1,A_2}\otimes\rho_{S_1}\otimes\rho_{S2}U_1^\dagger U_2^\dagger]
\end{align*}
with $U_k=e^{-i\hat{O}_{S_k}\otimes \hat{O}_{A_k}t}$. Writing $\hat{O}_{A_k}=\sum_i c_{A_k}^i\ket{c_{A_k}^i}\bra{c_{A_k}^i}$, the time evolved state can then be written as
\begin{align*}
    \rho_{S_1,S_2}(t)&=\sum_{i,j}\bra{c^i_{A_1},c^j_{A_2}}\rho_{A_1,A_2}\ket{c^i_{A_1},c^j_{A_2}}\times\\
    &e^{-i\hat{O}_{S_1} c^i_{A_1}t}\rho_{S_1}e^{i\hat{O}_{S_1} c^i_{A_1}t}\otimes e^{-i\hat{O}_{S_2}
    c^i_{A_2}t}\rho_{S_2}e^{i\hat{O}_{S_2} c^i_{A_2}t}.
\end{align*}
This is an expression of the form
\begin{align*}
    \sum_i p_i \rho_{S_1}'\otimes\rho_{S_2}'
\end{align*}
with $p_i$ a proper probably distribution. But this is a separable state and hence not entangled. Thus we have shown that a Hamiltonian of the form [\ref{eq:nonentanglinghamiltonian}] can not transfer entanglement from the ancillas to the system. \kfir{Actually we only showed that it can not begin transferring entanglement. The proof doesn't cover the case where the system starts out entangled. Also, it is easy to construct a stronger proof that shows both interactions must be greater than rank one}. 

